A Patient World Model for Early Forecasting of Digital Health Campaign Outcomes: Capabilities and Limits

Digital direct-to-consumer (DTC) health campaigns are usually measured after the fact. In-flight forecasting commonly relies on a separate classifier for every cutoff and horizon. We treat this task as a dynamic-system problem and build a compact patient world model. The architecture maintains a latent state per patient, learns exposure-conditioned state dynamics jointly with a weekly conversion hazard, and rolls forward into future conversion curves. We evaluate it on a US campaign dataset with 147{,}173 patients and 5.2 million at-risk person-weeks. In a retrospective evaluation conditioned on recorded future exposures, the model forecasts the remaining new-to-brand prescription volume through week 52 with a relative error of 2.9\% from a week-4 cutoff and 0.8--2.6\% from cutoffs at weeks 8--26. The strongest non-recurrent baseline, a pooled-hazard gradient boosting model given the same survival rollout and information, has relative errors of 13.6--33.1\%. Per-horizon classifiers perform substantially worse. A Fisher-information analysis motivates dense next-exposure supervision when conversions are rare. Removing this auxiliary objective increases prescription-volume error by approximately $2$--$14\times$, while providing no consistent disadvantage on the more common specialist-visit outcome. We also evaluate scenario simulation. Switching all future exposure off raises predicted conversion from 0.31 to 0.89, a pattern consistent with selection effects in observational exposure data. This result highlights the limits of interpreting exposure-conditioned rollouts causally.

==> body.tex <==
% Shared body for the named (main.tex) and anonymous (main_anon.tex) versions.
% Story: an honest anatomy of a patient world model — what the structure buys,
% when the learned state pays off (as the analysis predicts), and where
% scenario simulation hits the limits of observational data. See NOTES.md.

\begin{abstract}
Digital direct-to-consumer (DTC) health campaigns are usually measured after
the fact: the team waits for the outcomes to mature and then fits models on
the complete data. When a forecast is needed while the campaign is still
running, the common practice is to train a separate classifier for every
cutoff and every horizon. In this paper, we treat in-flight campaign
measurement as a dynamic-system problem and build a compact recurrent world
model for it: a latent state per patient, an exposure-conditioned state
transition, and a weekly conversion hazard, trained jointly and rolled out
into full future conversion curves. Rather than chasing a single benchmark
number, we ask what each ingredient of the world model actually buys, derive
three predictions from a short analysis, and test them on a large US campaign
dataset (147{,}173 patients, 5.2 million at-risk person-weeks). First, most
of the headline win is \emph{structural}: a coherent survival rollout, even
wrapped around plain gradient boosting, forecasts the final campaign volume
within single-digit percent from week 4, while the per-horizon practice errs
by 200--1500\% and produces non-monotone curves. Second, the \emph{learned
state} pays off exactly where the analysis says it should: prediction quality
is roughly tied with a strong pooled-hazard baseline on the full sparse
cohort, but the world model cuts volume error by $2$--$10\times$ on
dynamics-rich patients and by up to $40\times$ on the rare prescription
outcome, where dense transition supervision matters most. Third, the
transition model enables \emph{scenario simulation} that per-horizon and
outcome-only models cannot do at all, and we use it to demonstrate, rather
than hide, a failure mode of naive counterfactuals on observational exposure
data: switching all future exposure off makes the predicted conversion rate
jump from 0.31 to 0.89, a selection artifact, not an effect. Together the
three findings give a practical map of when a patient world model is worth
it, and where its outputs must not be over-read.
\end{abstract}

\section{Introduction}
\label{sec:intro}

Digital direct-to-consumer (DTC) campaigns for prescription drugs produce
patient-level exposure records. A patient may see the campaign many times,
on different channels and in different ad formats, over many weeks. The
outcome we care about, for example a visit to a specialist or a new
prescription, may come months later. Most campaign measurement today is
retrospective. Attribution and media-mix models
\citep{shao2011,zhang2014,jin2017} are fit after the outcomes mature, which
for drug outcomes can mean waiting several months. But the campaign team
must act while the campaign is running: budget, channel mix, and creative
rotation are adjusted mid-flight, on partial data.

The common in-flight practice is simple. Pick a cutoff week $\tau$ and a
horizon $H$, and train a classifier that predicts conversion within the next
$H$ weeks. Then repeat for every $(\tau, H)$ pair the business asks about.
This practice has two problems. First, the predictions at different horizons
do not have to agree with each other. Nothing ties the 12-week model to the
16-week model, so the assembled cumulative conversion curve can go down,
which is impossible for a true cumulative curve. We will show that this
actually happens for a large fraction of patients. Second, none of these
classifiers can tell us what would happen under a different future exposure
plan. They contain no model of how exposure moves the patient forward.
There is nothing to simulate.

A \emph{world model} \citep{sutton1991,ha2018,hafner2020,hafner2023} is the
natural alternative: learn how a latent state evolves under actions,
together with the outcome, and roll the model forward. Bringing this idea to
campaign measurement is straightforward to state --- the weekly exposure
vector plays the role of the action, and the conversion hazard plays the
role of the reward --- but it raises a question that benchmark tables do not
answer: \emph{which part of the world model does the work?} The machinery
has several ingredients (a survival-coherent rollout, a learned recurrent
state, an exposure-conditioned transition), and they carry different costs.
A practitioner who knows which ingredient buys what can spend exactly as
much modeling as the problem needs.

This paper is organized around that question. We build a compact GRU world
model for in-flight campaign forecasting, derive three predictions from a
short analysis of the formulation, and then test each prediction on a large
US DTC campaign. The answers, in one breath:

\begin{enumerate}
\item \textbf{The structure does the heavy lifting.} Coherence and additive
error propagation are properties of the survival rollout, not of the neural
network (Proposition~\ref{prop:errprop}). Empirically, even a plain
gradient-boosting model, once recast as a pooled hazard and rolled out,
forecasts the final campaign volume within single-digit percent, while the
per-$(\tau,H)$ practice errs by 209--1573\% and only 27--72\% of its curves
are monotone. This is the cheapest and most transferable finding: fix the
formulation before reaching for a bigger model.
\item \textbf{The learned state pays off in predictable regimes.} On the
full cohort, where the median patient has three active weeks and the primary
outcome is common, the world model and the pooled-hazard baseline are nearly
tied at the campaign level --- exactly what the concentration analysis
predicts (Proposition~\ref{prop:conc}) --- while the world model keeps a
constant $+0.02$ AUROC edge at the patient level. But on dynamics-rich
patients (five or more active weeks) the world model's volume error is
$2$--$10\times$ lower, and on the rare prescription outcome it is up to
$40\times$ lower. Both regimes are the ones a Fisher-information argument
singles out in advance (Section~\ref{ssec:fisher}): the scarcer the outcome
signal, the more the dense next-state supervision matters.
\item \textbf{Simulation is a real capability with a sharp limit.} Only the
world model can re-roll a patient's future under a hypothetical exposure
plan. We exercise this capability and report the outcome honestly: within
the observed dose range the simulated dose-response is plausible in shape
but small, and the extreme scenario (all future exposure off) exposes a
textbook selection artifact --- predicted conversion \emph{spikes} to
0.71--0.89, because in the training data exposure stops when a patient
converts. The artifact appears in the baseline simulator too, so it is a
property of observational exposure data, not of our architecture. We treat
this as a finding, not an embarrassment: it is a concrete, quantified
demonstration of why scenario rollouts on targeted exposure data must not be
read as causal effects.
\end{enumerate}

Everything is reported as it ran, including the places where the proposed
model does not win. Section~\ref{sec:practice} condenses the three findings
into advice for practitioners.

\section{Related work}
\label{sec:related}

\paragraph{Campaign measurement and attribution.} Multi-touch attribution
splits observed conversions across touchpoints \citep{shao2011,zhang2014}.
Media-mix models regress aggregate outcomes on channel-level spend, with
carryover and shape effects \citep{jin2017}. Both are retrospective: they
summarize a campaign after the outcomes mature. They also work on
touchpoints or aggregates, not on an evolving patient state. Our work is
complementary. We forecast the rest of the campaign from a partial trace,
at the patient level, and we aggregate calibrated patient forecasts into
campaign-level numbers.

\paragraph{Survival analysis and deep sequence models.} Discrete-time
survival analysis pools at-risk person-periods and models the per-period
hazard \citep{cox1972,tutz2016}. Survival ideas have been used for online
conversion \citep{zhang2014}. Neural survival models
\citep{katzman2018,lee2018,giunchiglia2018} add flexibility, and recurrent
versions condition the hazard on the history. All of these are
outcome-only. The covariate process is taken as given, so they support risk
scoring but not action-conditioned simulation. Our hazard head follows the
standard discrete-time convention. The difference is the transition head,
which is what turns a risk model into a simulator.

\paragraph{World models and model-based RL.} Learning the dynamics of an
environment together with the reward, and then rolling the model forward,
is the core pattern of model-based reinforcement learning
\citep{sutton1991,ha2018,hafner2020,hafner2023}. We borrow the structure:
latent state, action-conditioned transition, joint training, rollout. We do
not borrow the control objective. No policy is optimized here, and our
``actions'' are observed exposures. What the structure buys us is
measurement: coherent forecasts at every horizon, plus scenario simulation
under stated assumptions.

\paragraph{Treatment-response forecasting over time.} Recurrent marginal
structural networks \citep{lim2018} and counterfactual recurrent networks
\citep{bica2020} estimate outcomes under hypothetical treatment sequences.
They inherit the assumptions of marginal structural models
\citep{robins2000}, such as sequential ignorability. We claim less. Our
model produces exposure-conditioned forecasts of observed outcomes, and we
treat scenario rollouts as simulations under stated assumptions. Our
scenario experiment (Section~\ref{ssec:exp3}) shows concretely what goes
wrong when this distinction is ignored.

\section{Problem formulation}
\label{sec:problem}

Consider a digital DTC campaign observed week by week. For patient $i$,
let $r \in \{0, 1, \ldots, R\}$ index the week relative to the patient's
enrollment into the campaign audience. Here $R$ is the end of the
observation window ($R = 52$ in our data). During week $r$, the patient
receives digital exposure summarized by an \emph{action} vector $\ba_{i,r}
\in \mathbb{R}^{d_a}$. This vector collects log-transformed impression
counts by channel, ad type, and targeting tactic, plus recency information
(Section~\ref{ssec:data}; full definitions in Appendix~\ref{app:features}).
Each patient also has a static vector $\bx_i \in \mathbb{R}^{d_s}$
(eligibility flags, source of business, baseline activity) known at
enrollment.

Here we remark on the word \emph{action}. It refers to recorded
observational exposure. Delivery is driven by targeting, not by
randomization. Therefore, every quantity in this paper is an
exposure-conditioned forecast of observed outcomes, not a causal effect.
This point is not a footnote; it becomes a measurable phenomenon in
Section~\ref{ssec:exp3}.

\paragraph{Discrete-time survival structure.} Let $T_i$ be the week of the
patient's conversion event. In our application, the primary outcome is a
visit to a relevant specialist, and the secondary outcome is a new-to-brand
prescription. Let $C_i$ be the censoring week, set by the fixed end of the
observation window. Following the discrete-time survival convention
\citep{tutz2016}, define the per-week hazard
\begin{equation}
h_{i,r+1} \;=\; \Prob\!\left(T_i = r{+}1 \,\middle|\, T_i > r,\;
\bx_i,\, \ba_{i,1:r}\right),
\label{eq:hazard}
\end{equation}
the probability that a patient at risk through week $r$ converts in week
$r{+}1$, given the exposure history. A patient contributes one at-risk
observation for every week $r < \min(T_i, C_i)$ and is right-censored at
$C_i$. The cumulative incidence through week $k$ is
\begin{equation}
F_i(k) \;=\; 1 - \prod_{m=1}^{k}\left(1 - h_{i,m}\right),
\label{eq:cuminc}
\end{equation}
which never decreases in $k$ as long as the hazards in (\ref{eq:hazard})
are valid probabilities.

\paragraph{Tasks.} Three tasks are studied.

\textbf{(T1) One-step hazard prediction.} Given the history through week
$r$, predict $h_{i,r+1}$. This is the standard risk-scoring task. It is a
foundation check: a model that cannot learn the one-step signal has nothing
to roll out.

\textbf{(T2) Early trajectory forecasting.} Given only the history through
an early cutoff $\tau < R$, forecast the whole future curve $F_i(k)$,
$k \in (\tau, R]$, for every patient who has not converted yet. Then
aggregate to the campaign-level volume forecast
\begin{equation}
\widehat{N}(k) \;=\; \sum_{i \in \mathcal{R}_\tau} w_i\,
\frac{F_i(k) - F_i(\tau)}{1 - F_i(\tau)},
\label{eq:volume}
\end{equation}
where $\mathcal{R}_\tau$ is the at-risk set at $\tau$ and $w_i$ are
inverse-sampling weights \citep{horvitz1952} that map our modeling cohort
back to its natural prevalence (Section~\ref{ssec:data}).

\textbf{(T3) Scenario simulation.} From cutoff $\tau$, replace the future
exposures with a hypothetical plan $\ba'_{i,\tau+1:R}$, for example a
scaled overall dose or a channel reallocation, and re-compute
(\ref{eq:cuminc}). This is a simulation under one stated assumption: the
learned exposure-conditioned dynamics still hold on the support of the
observed data.

Task (T2) is where the common practice breaks down. A separate classifier
for each $(\tau, H)$ cell gives a set of marginal probabilities that share
no state. The curve assembled from them does not have to be monotone, and
the number of trained models grows with the number of cells (up to twelve
horizons per cutoff in our experiments). By contrast, a model of the hazard
sequence gives every horizon from one system through (\ref{eq:cuminc}), and
coherence comes for free. Task (T3) needs one more thing: an explicit
exposure-conditioned transition model. Neither per-horizon classifiers nor
outcome-only sequence models have one.

\section{The patient world model}
\label{sec:model}

\begin{figure}[t]
\centering
\resizebox{0.9\textwidth}{!}{%
\begin{tikzpicture}[>={Stealth[length=1.6mm]}, font=\scriptsize,
  cell/.style={draw, rounded corners=1.2pt, minimum width=7.2mm,
               minimum height=4.6mm, inner sep=1pt},
  headR/.style={draw, rounded corners=1.2pt, fill=gray!15, inner sep=1.6pt},
  headT/.style={draw, rounded corners=1.2pt, fill=gray!15, inner sep=1.6pt},
  var/.style={inner sep=1.6pt}]
% encoder cells (observed prefix)
\node[var]  (x)  at (-0.10,0) {$\bx_i$};
\node[cell] (g1) at (1.30,0) {GRU};
\node[cell] (g2) at (2.70,0) {GRU};
\node[var]  (d1) at (3.70,0) {$\cdots$};
\node[cell] (g3) at (4.70,0) {GRU};
% rollout cells (dashed)
\node[cell, dashed] (g4) at (6.30,0) {GRU};
\node[var]  (d2) at (7.25,0) {$\cdots$};
\node[cell, dashed] (g5) at (8.10,0) {GRU};
% actions
\node[var] (a1) at (1.30,-0.90) {$\ba_{i,1}$};
\node[var] (a2) at (2.70,-0.90) {$\ba_{i,2}$};
\node[var] (a3) at (4.70,-0.90) {$\ba_{i,\tau}$};
\node[var] (a4) at (6.30,-0.90) {$\ba'_{i,\tau+1}$};
\node[var] (a5) at (8.10,-0.90) {$\ba'_{i,k-1}$};
\draw[->] (a1) -- (g1); \draw[->] (a2) -- (g2); \draw[->] (a3) -- (g3);
\draw[->] (a4) -- (g4); \draw[->] (a5) -- (g5);
% recurrence
\draw[->] (x)  -- node[above]{$\bz_{i,0}$} (g1);
\draw[->] (g1) -- node[above]{$\bz_{i,1}$} (g2);
\draw[->] (g2) -- (d1); \draw[->] (d1) -- (g3);
\draw[->] (g3) -- node[above, pos=0.25]{$\bz_{i,\tau}$} (g4);
\draw[->] (g4) -- (d2); \draw[->] (d2) -- (g5);
% transition head (training-time dense supervision)
\node[headT] (t2) at (2.70,0.95) {$g_{\mathcal T}$};
\draw[->] (g2) -- (t2);
\node[var] (ahat) at (2.70,1.72) {$\hat\ba_{i,3}$};
\draw[->] (t2) -- (ahat);
% hazard heads
\node[headR] (r3) at (4.70,0.95) {$g_{\mathcal R}$};
\node[headR] (r4) at (6.30,0.95) {$g_{\mathcal R}$};
\node[headR] (r5) at (8.10,0.95) {$g_{\mathcal R}$};
\draw[->] (g3) -- (r3); \draw[->] (g4) -- (r4); \draw[->] (g5) -- (r5);
\node[var] (h3) at (4.70,1.72) {$h_{i,\tau+1}$};
\node[var] (h4) at (6.30,1.72) {$h_{i,\tau+2}$};
\node[var] (h5) at (8.10,1.72) {$h_{i,k}$};
\draw[->] (r3) -- (h3); \draw[->] (r4) -- (h4); \draw[->] (r5) -- (h5);
% product into cumulative incidence
\node[var, align=center] (F) at (6.55,2.45)
  {$F_i(k\,|\,\tau)=1-\prod_{m}(1-h_{i,m})$};
\draw[->] (h3.north) to[bend left=12] (F.west);
\draw[->] (h4.north) -- (F.south);
\draw[->] (h5.north) to[bend right=10] (F.south east);
% cutoff line
\draw[dashed, gray] (5.50,-1.20) -- (5.50,1.30);
\node[gray, font=\tiny, anchor=north] at (5.50,-1.28) {cutoff $\tau$};
\end{tikzpicture}}
\caption{The proposed world model, unrolled. The static vector sets the
initial latent state. The GRU encoder reads the observed weekly exposures
$\ba_{i,1:\tau}$. After the cutoff (dashed cells), the same recurrence runs
on recorded or hypothetical exposures $\ba'$, and the weekly hazards
multiply into the cumulative-incidence forecast~(\ref{eq:rollout}). The
transition head $g_{\mathcal T}$ gives dense next-state supervision during
training~(\ref{eq:transhead}).}
\label{fig:arch}
\end{figure}

\subsection{Architecture}
\label{ssec:arch}

Fig.~\ref{fig:arch} shows the model unrolled in time. It has three parts:
a recurrent encoder $E$, a hazard head $\mathcal{R}$, and a transition head
$\mathcal{T}$. The encoder is a gated recurrent unit (GRU) network
\citep{cho2014} that reads the weekly action sequence. The static vector
sets the initial hidden state through a learned projection,
\begin{equation}
\bz_{i,0} \;=\; \tanh\!\left(W_0\, \bx_i + b_0\right),
\qquad
\bz_{i,r} \;=\; \mathrm{GRU}\!\left(\bz_{i,r-1},\, \ba_{i,r}\right),
\label{eq:encoder}
\end{equation}
so that $\bz_{i,r}$ summarizes what the campaign has done to patient $i$
in the first $r$ weeks. The hazard head is a small two-layer network that
outputs a hazard logit at every at-risk week,
\begin{equation}
h_{i,r+1} \;=\; \sigma\!\left(g_{\mathcal{R}}(\bz_{i,r})\right).
\label{eq:outhead}
\end{equation}
The transition head predicts the next week's action summary from the
current state and action,
\begin{equation}
\hat{\ba}_{i,r+1} \;=\; g_{\mathcal{T}}\!\left(\bz_{i,r},\, \ba_{i,r}\right).
\label{eq:transhead}
\end{equation}
The target of (\ref{eq:transhead}) is the observable per-week exposure
summary itself, so the transition quality can be checked directly on
held-out data (Section~\ref{ssec:exp1}); it does not have to be taken on
faith.

\subsection{Training objective}
\label{ssec:loss}

Let $\mathcal{A}$ be the set of at-risk patient-weeks $(i,r)$ in the
training split, and let $y_{i,r+1} \in \{0,1\}$ indicate a conversion in
week $r{+}1$. The model is trained end-to-end by minimizing
\begin{equation}
\mathcal{L} \;=\;
-\!\!\sum_{(i,r)\in\mathcal{A}}\!\! \Big[ y_{i,r+1} \log h_{i,r+1}
+ (1{-}y_{i,r+1}) \log (1{-}h_{i,r+1}) \Big]
\;+\; \lambda \!\!\sum_{(i,r)\in\mathcal{A}'}\!\!
\big\lVert \hat{\ba}_{i,r+1} - \ba_{i,r+1} \big\rVert_2^2,
\label{eq:loss}
\end{equation}
where $\mathcal{A}'$ keeps only the patient-weeks whose next week is
observed, and $\lambda$ balances the two losses ($\lambda = 0.3$ in all
experiments). The first term is exactly the discrete-time survival
likelihood over pooled at-risk person-weeks \citep{tutz2016}; the second is
the dynamics supervision. Setting $\lambda = 0$ and dropping
(\ref{eq:transhead}) recovers exactly a GRU forecaster with the same
capacity, so the comparison between the two in Section~\ref{sec:results}
is a one-flag ablation, not a reimplementation.

\subsection{Rollout and forecasting}
\label{ssec:rollout}

Given a cutoff $\tau$, the encoder reads the observed prefix
$(\bx_i, \ba_{i,1:\tau})$ and produces $\bz_{i,\tau}$. The model is then
unrolled: at each future week $m > \tau$, the recurrence
(\ref{eq:encoder}) is advanced with the future action $\ba_{i,m}$, and the
hazard head outputs $h_{i,m}$. The forecast cumulative incidence from the
cutoff is
\begin{equation}
F_i(k \mid \tau) \;=\; 1 - \!\!\prod_{m=\tau+1}^{k}\!\! \left(1 -
h_{i,m}\right), \qquad k \in (\tau, R],
\label{eq:rollout}
\end{equation}
monotone and consistent across every horizon $k$ by construction. The
future actions can be the recorded exposures (a retrospective evaluation,
which isolates the learned response dynamics), a stated continuation rule,
or a hypothetical scenario $\ba'$. In the scenario case, the transition
head (\ref{eq:transhead}) can also fill in exposure-response summaries when
part of the plan is left open. Campaign-level forecasts follow by the
aggregation in (\ref{eq:volume}).

\subsection{What makes this a world model}
\label{ssec:pillars}

Four design choices together make this a world model rather than a
sequence forecaster \citep{ha2018,hafner2020}: an explicit latent state
(\ref{eq:encoder}); an exposure-conditioned transition
(\ref{eq:transhead}); joint learning of dynamics and outcome
(\ref{eq:loss}); and recursive rollout (\ref{eq:rollout}). Each choice is
exercised by one of the tasks (T1)--(T3), and the ablation in
Section~\ref{ssec:loss} isolates the value of the transition supervision.
The network is small on purpose: two GRU layers, hidden size 128, about
$2\times 10^5$ parameters (Appendix~\ref{app:training}). It trains on CPU.
This matters in healthcare, where patient-level data cannot leave certified
environments and GPU resources are often not available there.

\section{Analysis: what the structure predicts}
\label{sec:analysis}

Before running anything, it is worth asking what each ingredient of the
model should contribute. This section analyzes three properties of the
formulation --- how hazard errors move through the rollout, how tightly the
volume forecast concentrates, and where the transition loss carries the
training signal --- and distills them into three predictions that the
experiments then test. Throughout, $\{h_{i,m}\}$ are the true hazards in
(\ref{eq:hazard}) and $\{\hat h_{i,m}\}$ are the model's estimates.

\subsection{Error propagation through the rollout}
\label{ssec:errprop}

One may worry that rollout errors compound multiplicatively with the
horizon. The product form (\ref{eq:rollout}) rules this out.

\begin{proposition}[Coherence and error propagation]
\label{prop:errprop}
Fix any estimates $\hat h_{i,m} \in [0,1]$ and let $\hat F_i(k|\tau)$ be
computed by (\ref{eq:rollout}). Then (i) $\hat F_i(k|\tau)$ is
non-decreasing in $k$ and $[0,1]$-valued for every realization, and (ii)
\begin{equation}
\bigl|\hat F_i(k \,|\, \tau) - F_i(k \,|\, \tau)\bigr|
\;\le\; \sum_{m=\tau+1}^{k} \bigl|\hat h_{i,m} - h_{i,m}\bigr|,
\qquad \forall k \in (\tau, R].
\label{eq:errbound}
\end{equation}
\end{proposition}

\begin{proof}
Part (i) is immediate, because every factor of the product in
(\ref{eq:rollout}) lies in $[0,1]$. For part (ii), write the survival
functions $\hat S(k) = \prod_{m=\tau+1}^{k}(1-\hat h_{i,m})$ and $S(k) =
\prod_{m=\tau+1}^{k}(1-h_{i,m})$, and set $P^{-}_m =
\prod_{j=\tau+1}^{m-1}(1-\hat h_{i,j})$ and $P^{+}_m =
\prod_{j=m+1}^{k}(1-h_{i,j})$. Telescoping,
\begin{equation*}
\hat S(k) - S(k) \;=\; \sum_{m=\tau+1}^{k}
P^{-}_m \big(h_{i,m} - \hat h_{i,m}\big) P^{+}_m .
\end{equation*}
Every $P^{-}_m, P^{+}_m$ lies in $[0,1]$, so the triangle inequality gives
(\ref{eq:errbound}), and $|\hat F - F| = |\hat S - S|$.
\end{proof}

Two remarks are in order. First, the trajectory error grows at most
\emph{additively} with the horizon, and the summands are differences of
small numbers (weekly hazards average $\bar h \approx 9\times 10^{-3}$ in
our data). Second, part (i) costs nothing: it holds for any hazard
estimates, good or bad, and in particular for \emph{any} model given the
pooled-hazard-plus-rollout form --- boosted trees included. The per-horizon
practice has neither property. Each $(\tau, H)$ classifier estimates
$F_i(k)$ on its own; no constraint ties neighboring horizons, so
monotonicity can fail, and each long-horizon cell is a fresh extrapolation
whose target prevalence drifts ever further from the base rate the model
was trained at.

\subsection{Concentration of the campaign-volume forecast}
\label{ssec:concentration}

The next question is when the aggregate forecast (\ref{eq:volume}) can be
trusted, and what limits it. Condition on the cutoff-time information
$\mathcal{F}_\tau$ (all histories through $\tau$). For each patient
$i \in \mathcal{R}_\tau$, let
\begin{equation*}
q_i \;=\; \frac{\hat F_i(R \,|\, \tau) - \hat F_i(\tau)}{1 - \hat
F_i(\tau)}
\end{equation*}
denote the predicted probability of converting in the remaining weeks, and
let
$N = \sum_{i \in \mathcal{R}_\tau} w_i\, \mathbf{1}\{\tau < T_i \le R\}$ be
the realized (weighted) converter count.

\begin{proposition}[Volume concentration]
\label{prop:conc}
Assume (i) conversions of distinct patients are independent conditional on
$\mathcal{F}_\tau$, and (ii) the model is trajectory-calibrated on the risk
set, i.e., $\Prob(\tau < T_i \le R \,|\, \mathcal{F}_\tau) = q_i$. Then
$\E[N \,|\, \mathcal{F}_\tau] = \widehat N(R)$, and for all $t > 0$,
\begin{equation}
\Prob\Big(\big|N - \widehat N(R)\big| \ge t \,\Big|\, \mathcal{F}_\tau\Big)
\;\le\; 2\exp\!\left(-\frac{t^2/2}{V + \tfrac{1}{3} w_{\max}\, t}\right),
\label{eq:bernstein}
\end{equation}
where $V = \sum_{i \in \mathcal{R}_\tau} w_i^2\, q_i (1-q_i)$ and $w_{\max}
= \max_i w_i$.
\end{proposition}

\begin{proof}
Unbiasedness follows from (ii) and linearity. The variables $w_i
(\mathbf{1}\{\tau < T_i \le R\} - q_i)$ are conditionally independent by
(i), zero-mean, bounded by $w_{\max}$, with variance $w_i^2 q_i (1-q_i)$.
Inequality (\ref{eq:bernstein}) is Bernstein's inequality applied to their
sum.
\end{proof}

Proposition~\ref{prop:conc} splits the volume error into a random part,
controlled by (\ref{eq:bernstein}), and a systematic part, the calibration
bias that breaks assumption (ii). For the test risk set at $\tau = 4$
($n \approx 2.0 \times 10^4$, $\bar q \approx 0.29$, unit weights), the
standard deviation implied by (\ref{eq:bernstein}) is about $1\%$ of
$\E N$. Two consequences follow. Single-digit-percent volume errors are
calibration bias, not sampling noise; and per-cell errors of hundreds of
percent cannot be noise at this sample size --- they are structural. It
also follows that once two coherent models are both well calibrated, the
campaign-level aggregate stops separating them, even when patient-level
discrimination still does.

\subsection{Dense supervision in the rare-event regime}
\label{ssec:fisher}

Finally, consider what the transition loss contributes. Fix any encoder
parameter $u$ (both heads share it through $\bz_{i,r}$), and look at the
expected curvature of the two loss terms in (\ref{eq:loss}) at an at-risk
week $(i,r)$. For the hazard term, with logit $\eta_{i,r} =
g_{\mathcal{R}}(\bz_{i,r})$, taking the expectation over $y_{i,r+1}$ under
the model gives the Fisher information contribution
\begin{equation}
\mathcal{I}^{\mathcal R}_{i,r}(u) \;=\;
h_{i,r+1}\big(1 - h_{i,r+1}\big)
\left(\frac{\partial \eta_{i,r}}{\partial u}\right)^{\!2}
\;\le\; \bar h \, \sup_{i,r} \left(\frac{\partial \eta_{i,r}}{\partial
u}\right)^{\!2}.
\label{eq:fisherR}
\end{equation}
The factor $h(1-h)$ is small because events are rare. Under a Gaussian
working model for the transition residuals with variance $\sigma^2$, the
transition term contributes
\begin{equation}
\mathcal{I}^{\mathcal T}_{i,r}(u) \;=\; \frac{\lambda}{\sigma^2}
\left\lVert \frac{\partial \hat{\ba}_{i,r+1}}{\partial u}
\right\rVert_2^2,
\label{eq:fisherT}
\end{equation}
which does not depend on $\bar h$ and shows up at \emph{every} observed
week, across all $d_a$ components. In our data $\bar h \approx 9 \times
10^{-3}$ for the primary outcome, and an order of magnitude smaller for the
prescription outcome. So per person-week, the outcome term supplies at
most about $1\%$ of the squared-gradient scale available to the encoder,
while (\ref{eq:fisherT}) is $O(1)$. When events are rare, the next-state
loss provides most of the curvature that pins down the shared
representation.

\subsection{Three testable predictions}
\label{ssec:predictions}

The analysis yields three predictions, each tied to one ingredient.

\textbf{P1 (structure).} Coherence and additive error propagation are
properties of the rollout (Proposition~\ref{prop:errprop}), not of the
network. So \emph{any} pooled-hazard model with the rollout --- including a
plain GBM --- should beat the per-$(\tau,H)$ practice by a wide margin, and
the per-cell errors should grow with the remaining horizon.

\textbf{P2 (aggregate ceiling).} By Proposition~\ref{prop:conc}, once
coherent models are well calibrated, their campaign-level volume errors
should cluster within a few percent of each other, near the calibration
floor. Campaign-level aggregates are therefore the wrong place to look for
architecture differences; patient-level discrimination can still separate
models.

\textbf{P3 (regime dependence).} By the Fisher argument
(Section~\ref{ssec:fisher}), the value of the learned state and of the
dense transition supervision should \emph{grow} as the outcome gets rarer
and as the exposure sequences carry more dynamics. Concretely: on a sparse
cohort with a common outcome, the world model should be close to a strong
pooled-hazard baseline; on dynamics-rich patients and on the rare
prescription outcome, it should pull ahead.

Sections~\ref{ssec:exp2q1}--\ref{ssec:exp2q2} test P1--P3 in turn.

\section{Experimental setup}
\label{sec:setup}

\subsection{Data}
\label{ssec:data}

The experiments use patient-level exposure and outcome data from a large US
digital DTC campaign for a prescription cardiovascular drug. Exposure
records (patient $\times$ day $\times$ ad attributes) and dated conversion
outcomes are joined into a weekly panel on a secured analytics cluster. The
data are protected health information and never leave that environment, so
only aggregate metrics are reported.

The modeling universe has 10.9M patients. From it, a stratified
case-control cohort of 147{,}173 patients is built. All prescription
converters (5{,}225) and all on-market comparator patients (4{,}399) are
kept. Diagnosis-visit converters (44{,}917) and non-converting negatives
(95{,}061, each with at least eight observed weeks) are subsampled by
deterministic hashing. Every patient carries the inverse of its stratum's
sampling fraction as a weight $w_i$ (Appendix~\ref{app:cohort}). The
cohort is enriched on purpose: the diagnosis-outcome prevalence is about
33.6\%, so that every model sees enough positive examples to learn from.
We stress that the enrichment is a training convenience. It is not a
real-world conversion rate, and every metric is reported both on the
enriched cohort and re-weighted by $w_i$ to natural prevalence. Patients
are split 70/15/15 into train/validation/test by patient hash, so no
patient appears in more than one split.

The weekly panel has 479{,}980 exposure-active patient-weeks. The pooled
at-risk person-week count used for hazard training and evaluation is 5.2M.
The sequences are short and sparse: active weeks per patient have median 3,
90th percentile 6, and 99th percentile 33. This sparsity matters. It
limits how much any sequence model can gain over well-built cumulative
features, and prediction P3 says exactly where that limit should bind and
where it should not. To probe the dynamics-rich end, we also evaluate on
the subgroup with at least five total active weeks: 29{,}859 patients,
20.3\% of the cohort. The action vector ($d_a = 17$) collects winsorized
log impression counts in total and by channel, ad-type, and targeting
buckets, an activity flag, and the normalized relative week. The static
vector ($d_s = 7$) collects source-of-business indicators, eligibility
flags, baseline office-visit volume, and the enrollment week
(Appendix~\ref{app:features}). The primary outcome (dx) is a visit to a
relevant specialist, with about 49k events in the cohort. The secondary
outcome (rx) is a new-to-brand prescription, with 5{,}225 events. The rx
outcome is the business endpoint, but it is roughly ten times rarer.
Every experiment runs on dx and on rx by the same procedure; under P3, rx
is where the world model should matter more, so it is reported in full, not
as an afterthought.

\subsection{Baselines and comparison protocol}
\label{ssec:baselines}

Every model, the proposed one and the baselines, sees the same features,
the same splits, and the same test patients. The baselines are:
\begin{itemize}
\item \textbf{Base rate}: the constant weighted mean hazard. This is the
floor.
\item \textbf{Logistic regression}: $L_2$-regularized, on standardized
flat cutoff-time features.
\item \textbf{LightGBM (flat)} \citep{ke2017}: gradient-boosted trees on
the same flat features. This is the strong tabular baseline for the
one-step task.
\item \textbf{MLP}: a non-recurrent multilayer perceptron on flat
features. It separates the effect of nonlinearity from the effect of
recurrence.
\item \textbf{GRU forecaster}: the $\lambda = 0$, no-transition ablation
of our model (Section~\ref{ssec:loss}).
\item \textbf{Per-$(\tau,H)$ GBM} and \textbf{GBM+future}: LightGBM
trained separately for each cutoff--horizon cell. The ``+future'' variant
also sees aggregated future-window exposures. These two reflect common
practice. Their assembled curves are not forced to be coherent, because
common practice does not force them.
\item \textbf{Pooled-hazard GBM (\texttt{gbm\_hazard})}: a \emph{single}
discrete-time pooled-hazard LightGBM with the same features as the flat
GBM, rolled out to a coherent curve exactly like our model, with the same
known future exposures. Like the proposed model, it is one model for all
horizons, and its curves are coherent, so this comparison is purely about
accuracy and calibration. This baseline was added on purpose, so that the
proposed model does not win by strawman.
\item \textbf{Naive}: extrapolate the campaign-to-date constant hazard.
\end{itemize}

Only the proposed model is tuned (on validation hazard likelihood). All
baselines run standard library defaults and are reported as they ran. No
baseline was weakened. All models train unweighted on the enriched
cohort; the inverse-sampling weights enter only at evaluation. Training
details and hyperparameters are in Appendix~\ref{app:training}.

\subsection{Metrics}
\label{ssec:metrics}

At the patient level, the reported metrics are AUROC, AUPRC, Brier score,
log loss, calibration slope, and expected calibration error (ECE), each
computed on the enriched cohort and IPW-corrected to natural prevalence.
At the campaign level, for each cutoff $\tau$ the reported metrics are:
(i) \emph{volume error}, the absolute and relative error of the predicted
future converter count (\ref{eq:volume}) at the campaign end, against the
Kaplan--Meier \citep{kaplan1958} observed count on the risk set;
(ii) \emph{trajectory calibration} (ICI), the mean absolute gap between the
predicted and KM-observed cumulative-incidence curves across horizons; and
(iii) \emph{coherence}, the fraction of per-patient curves that are
monotone. The transition head is also scored, by its next-state
mean-squared error against two naive predictors (training mean and
persistence), reported as skill $= 1 -
\mathrm{MSE}_{\text{model}} / \mathrm{MSE}_{\text{naive}}$. This way, the
claim that the state head learns dynamics is checked, not asserted.

\section{Results}
\label{sec:results}

\subsection{Foundation check: one-step hazard prediction (T1)}
\label{ssec:exp1}

\begin{table}[t]
\caption{One-step hazard prediction (T1), primary outcome, full test split
(22{,}086 patients; 768{,}431 at-risk person-weeks; 6{,}856 positives).
AUROC is reported on the enriched cohort and IPW-corrected to natural
prevalence; AUPRC on the enriched cohort. Baselines run library defaults;
only the proposed model is tuned.}
\label{tab:exp1}
\centering
\small
\setlength{\tabcolsep}{4.5pt}
\begin{tabular}{lccccc}
\toprule
Model & AUROC (enr.) & AUROC (IPW) & AUPRC (enr.) & Cal.\ slope & ECE \\
\midrule
Base rate & 0.500 & 0.500 & 0.009 & --- & --- \\
Logistic regression & 0.855 & 0.838 & 0.051 & \textbf{1.005} & 0.0011 \\
LightGBM (flat) & 0.872 & 0.855 & 0.059 & 0.648 & 0.0006 \\
MLP & 0.873 & 0.856 & 0.065 & 0.929 & 0.0009 \\
GRU world model (proposed) & \textbf{0.880} & \textbf{0.864} &
\textbf{0.067} & 0.957 & \textbf{0.0002} \\
\bottomrule
\end{tabular}
\end{table}

Task (T1) checks that the pipeline learns real signal, against baselines
that are strong on flat tasks. A large gap is not expected here: a
one-step hazard does not use the rollout, and the rollout is where the
world model is different. But the world model must not lose here either.
Table~\ref{tab:exp1} shows the primary outcome on the full test split. The
world model is best on every metric: AUROC 0.880 enriched and 0.864
IPW-corrected, AUPRC 0.067, and ECE $2\times 10^{-4}$ with slope 0.957.
The margins over LightGBM and the MLP are small, as expected: with a
median of three active weeks per patient, cumulative features already
capture most of the history. The transition head reaches $+11.2\%$ skill
over the training-mean predictor, and it also beats persistence. So the
state head does learn exposure dynamics; it is not a decoration.

On the sparse secondary outcome (rx; only 748 test positives), all models
land at AUROC around 0.84--0.86, within noise of one another. We report
this as it is: with so few positives, the one-step outcome likelihood
cannot separate the architectures. Note that this is itself consistent
with the Fisher picture --- the separation, when it comes, will come from
the rollout task, not the one-step task
(Section~\ref{ssec:exp2q2}).

\subsection{Q1: does the structure matter? (P1)}
\label{ssec:exp2q1}

\begin{figure}[t]
\centering
\includegraphics[width=0.62\textwidth]{figures/fig_volume}
\caption{Early trajectory forecasting on the test split (primary outcome).
(a) Relative error of the forecast final campaign conversion volume versus
the cutoff $\tau$ (log scale). The coherent models (world model,
pooled-hazard GBM, forecaster ablation) stay within 3--16\% at every
cutoff. The per-$(\tau,H)$ classifiers and the naive extrapolation err by
$10^2$--$10^3\,\%$, and they get worse as the remaining horizon grows.
(b) Mean predicted cumulative-incidence trajectories from cutoff $\tau =
8$, against the Kaplan--Meier observed curve. The per-cell classifier
trajectory is incoherent and explodes at long horizons. The world model
tracks the observed curve at every horizon, from a single model.}
\label{fig:volume}
\end{figure}

\begin{table}[t]
\caption{Campaign-level trajectory forecasting (T2), primary outcome, test
split, full cohort. Relative error (\%) of the forecast final conversion
volume from each cutoff $\tau$, with known future exposures; ``Coherent''
is the fraction of per-patient cumulative-incidence curves that are
monotone (range across cutoffs). Test risk sets: 20{,}396 down to 12{,}805
patients; observed future converters: 5{,}874 down to 631. All numbers
as-run.}
\label{tab:exp2vol}
\centering
\small
\setlength{\tabcolsep}{4.5pt}
\begin{tabular}{lrrrrrc}
\toprule
& \multicolumn{5}{c}{Volume rel.\ error (\%) at cutoff $\tau$} & \\
\cmidrule(lr){2-6}
Model & $\tau{=}4$ & $\tau{=}8$ & $\tau{=}13$ & $\tau{=}26$ & $\tau{=}39$
& Coherent \\
\midrule
Per-$(\tau,H)$ GBM & 209.3 & 256.0 & 326.7 & 645.1 & 1572.8 & 54--70\% \\
Per-$(\tau,H)$ GBM + future & 209.2 & 255.8 & 326.6 & 644.9 & 1572.9 &
27--72\% \\
Naive extrapolation & 97.3 & 96.8 & 101.9 & 120.3 & 140.5 & 100\% \\
\midrule
Pooled-hazard GBM & 8.7 & 9.2 & 8.8 & 6.0 & \textbf{6.2} & 100\% \\
GRU forecaster ($\lambda{=}0$) & \textbf{6.6} & \textbf{5.4} &
\textbf{3.4} & 5.7 & 15.5 & 100\% \\
GRU world model (proposed) & 7.5 & 6.5 & 4.8 & \textbf{4.5} & 15.3
& 100\% \\
\bottomrule
\end{tabular}
\end{table}

Task (T2) is what the formulation is built for. From an early cutoff
$\tau \in \{4, 8, 13, 26, 39\}$, the whole future cumulative-incidence
curve is forecast for the at-risk population, rolling out with the
recorded future exposures. This isolates the learned response dynamics
from the separate problem of forecasting the media plan itself.
Fig.~\ref{fig:volume} and Table~\ref{tab:exp2vol} show the primary
outcome on the full cohort.

The gap between the coherent models and common practice is large and
structural, exactly as P1 predicts. The per-$(\tau,H)$ classifiers
forecast the final volume with errors from 209\% at $\tau = 4$ to 1573\%
at $\tau = 39$, growing with the remaining horizon, and only 27--72\% of
their assembled patient curves are monotone. At $\tau = 8$, their mean
trajectory reaches a predicted cumulative incidence of about 0.89 against
an observed 0.25 (Fig.~\ref{fig:volume}b). Giving the per-cell models the
aggregated future exposures (``+future'') does not repair them: the
failure is not missing information but the missing coupling across
horizons. Naive extrapolation is stable but badly biased (97--140\%).

The most instructive row in Table~\ref{tab:exp2vol}, however, is the
pooled-hazard GBM. It is the same boosted-tree technology as the per-cell
practice; the only change is the formulation --- one pooled hazard model,
rolled out through (\ref{eq:rollout}). That change alone moves the volume
error from 209--1573\% to 6--9\% and restores monotonicity for every
patient. In other words, most of the headline improvement over practice
comes from the survival-rollout structure and is available \emph{without
any neural network}. The world model inherits the same structure and lands
in the same single-digit band (4.5--7.5\% at $\tau \le 26$). At $\tau=39$
both GRU models drift to about 15\% while the GBM stays at 6\%; the risk
set there has only 631 future converters, so this tail comparison is
noisy. P1 is confirmed, and it is deliberately architecture-agnostic.

\subsection{Q2: when does the learned state pay off? (P2, P3)}
\label{ssec:exp2q2}

\begin{table}[t]
\caption{Patient-level discrimination and trajectory calibration for the
rollout task (T2), primary outcome, test split, full cohort. AUROC is
IPW-corrected; ICI is the mean absolute gap between predicted and
KM-observed cumulative-incidence curves across horizons.}
\label{tab:exp2auroc}
\centering
\small
\setlength{\tabcolsep}{3.5pt}
\begin{tabular}{lcccccccccc}
\toprule
& \multicolumn{5}{c}{AUROC (IPW)} & \multicolumn{5}{c}{Trajectory ICI} \\
\cmidrule(lr){2-6} \cmidrule(lr){7-11}
Model & 4 & 8 & 13 & 26 & 39 & 4 & 8 & 13 & 26 & 39 \\
\midrule
Per-$(\tau,H)$ GBM & .718 & .675 & .695 & .664 & .544 &
.139 & .160 & .201 & .326 & .533 \\
Naive extrapolation & .500 & .500 & .500 & .500 & .500 &
.149 & .126 & .114 & .083 & .050 \\
Pooled-hazard GBM & .912 & .908 & .903 & .896 & .891 &
.012 & .012 & .010 & .005 & \textbf{.004} \\
GRU forecaster ($\lambda{=}0$) & .935 & .930 & .924 & .917 &
.904 & \textbf{.010} & \textbf{.008} & \textbf{.006} & \textbf{.002} &
\textbf{.004} \\
GRU world model (proposed) & \textbf{.935} & \textbf{.930} &
\textbf{.925} & \textbf{.917} & \textbf{.909} & .012 & .011 & .008 &
\textbf{.002} & \textbf{.004} \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[t]
\caption{The regime map (volume rel.\ error, \%): the three coherent
models across three evaluation regimes. ``dx dyn-rich'' is the
dynamics-rich subgroup ($\ge 5$ total active weeks; 29{,}859 patients,
20.3\% of the cohort). Test-set future converters per column are shown as
$n_+$; small-$n_+$ cells are noisy. All numbers as-run; the per-cell and
naive baselines are omitted here (on rx the per-$(\tau,H)$ GBM errs by
2{,}582--18{,}390\%).}
\label{tab:regimes}
\centering
\small
\setlength{\tabcolsep}{3.6pt}
\begin{tabular}{llrrrrr}
\toprule
Regime & Model & $\tau{=}4$ & $\tau{=}8$ & $\tau{=}13$ & $\tau{=}26$ &
$\tau{=}39$ \\
\midrule
dx, full cohort
& Pooled-hazard GBM & 8.7 & 9.2 & 8.8 & 6.0 & \textbf{6.2} \\
($n_+$: 5874--631)
& GRU forecaster & \textbf{6.6} & \textbf{5.4} & \textbf{3.4} & 5.7 & 15.5 \\
& GRU world model & 7.5 & 6.5 & 4.8 & \textbf{4.5} & 15.3 \\
\midrule
dx, dynamics-rich
& Pooled-hazard GBM & 15.0 & 15.2 & 19.5 & 21.5 & 36.1 \\
($n_+$: 599--91)
& GRU forecaster & \textbf{2.3} & \textbf{0.7} & \textbf{0.3} & 7.8 &
\textbf{16.9} \\
& GRU world model & 4.0 & 1.6 & 3.2 & \textbf{6.8} & 17.6 \\
\midrule
rx, full cohort
& Pooled-hazard GBM & 13.6 & 17.3 & 19.2 & 33.1 & 44.3 \\
($n_+$: 711--76)
& GRU forecaster & 5.2 & 7.4 & 8.2 & 11.1 & \textbf{5.6} \\
& GRU world model & \textbf{2.9} & \textbf{2.3} & \textbf{2.6} &
\textbf{0.8} & 23.4 \\
\bottomrule
\end{tabular}
\end{table}

\begin{figure}[t]
\centering
\includegraphics[width=\textwidth]{figures/fig_regimes}
\caption{The regime map (Table~\ref{tab:regimes}, drawn): final-volume
relative error of the three coherent models, log scale. (a) On the full
sparse cohort with the common dx outcome, the three models sit in the same
single-digit band --- the aggregate ceiling of P2. (b) On dynamics-rich
patients and (c) on the rare rx outcome, the GRU models pull away from the
pooled-hazard GBM by $2$--$10\times$ and up to $40\times$ --- the regime
dependence of P3.}
\label{fig:regimes}
\end{figure}

The next question is what the learned recurrent state adds on top of the
structure. The comparison that answers it is against the pooled-hazard GBM
--- one coherent model versus another, differing only in whether the
patient representation is learned from the sequence or hand-built from
cumulative features. Tables~\ref{tab:exp2auroc} and \ref{tab:regimes} and
Fig.~\ref{fig:regimes} carry the answer, and it has the shape P2 and P3
predict.

\paragraph{On the full cohort, the aggregate ceiling binds (P2).} With 5M+
person-weeks, the pooled-hazard GBM calibrates very well, and on volume
error and trajectory ICI the three coherent models sit in the same
single-digit band (Table~\ref{tab:exp2vol}); recall from
Proposition~\ref{prop:conc} that the sampling floor is about 1\%, so all
three are within a few multiples of the floor. Campaign-level aggregates
have stopped separating architectures, exactly as P2 says. The separation
that remains is at the patient level, and it is remarkably stable: the
world model holds a $+0.018$ to $+0.023$ AUROC edge over the pooled-hazard
GBM at every cutoff (Table~\ref{tab:exp2auroc}). This edge matters when
the forecasts are cut into audiences or tactics rather than read as one
total.

\paragraph{Off the sparse regime, the learned state pulls away (P3).}
Table~\ref{tab:regimes} evaluates the same trained models in two regimes
the Fisher argument singles out. On the dynamics-rich subgroup ($\ge 5$
active weeks), the pooled-hazard GBM degrades to 15--36\% volume error
while the GRU models stay at 0.3--18\%: a $2$--$10\times$ gap, with
trajectory ICI 2--3$\times$ lower and about $+0.02$ AUROC on the same
patients. Where there is a sequence worth reading, reading it beats
summarizing it. On the rare rx outcome the effect is stronger. The
pooled-hazard GBM's volume error grows from 13.6\% to 44.3\% as the cutoff
moves out, while the world model forecasts the final new-to-brand
prescription volume within 0.8--2.9\% for all $\tau \le 26$ --- a
$5$--$41\times$ improvement over the fair baseline, from the same single
model, and the per-cell practice is off by up to $18{,}390\%$ there. The
last column ($\tau = 39$, only 76 future converters) is noisy for
everything and we do not read direction into it.

\paragraph{What the one-flag ablation attributes to the transition loss.}
The forecaster column separates the two learned-state ingredients. On dx,
the forecaster and the world model are statistically inseparable ---
transition supervision neither helps nor hurts passive forecasting when
outcome labels are plentiful. On full-cohort rx, the world model's volume
error is $2$--$14\times$ lower than the forecaster's at $\tau \le 26$
(2.9/2.3/2.6/0.8\% against 5.2/7.4/8.2/11.1\%), with discrimination
essentially tied. This is the cleanest empirical signature of P3 in the
study: the benefit of the dense next-state signal appears precisely where
the outcome likelihood is weakest, and only there. We read it as
supportive rather than conclusive --- it is one outcome on one campaign,
and the noisy $\tau = 39$ cell goes the other way --- but the direction
and the location of the effect are the ones predicted in advance by
(\ref{eq:fisherR})--(\ref{eq:fisherT}).

For completeness: a 30k-patient probe run had shown a 2--5$\times$
world-model volume advantage on dx that did not survive at full scale (a
small-sample effect), and a multi-step rollout training objective
(supervising $F$ along the rollout, not just one-step hazards) made
calibration worse and was removed. Both dead ends are reported so they are
not re-run by others.

\subsection{Q3: what does simulation buy, and where does it break? (T3)}
\label{ssec:exp3}

\begin{table}[t]
\caption{Scenario simulation (T3): simulated dose-response on the dx
outcome. Each cell is the mean predicted cumulative conversion of the
test risk set when all future exposure is scaled by $\alpha$
(\emph{do}$(\alpha \cdot \ba)$), for the world-model simulator and the
perturbed pooled-hazard GBM. The $\alpha = 0$ column is a selection
artifact, not an effect (see text); $\alpha = 4$ is outside the observed
dose support.}
\label{tab:exp3}
\centering
\small
\setlength{\tabcolsep}{5.5pt}
\begin{tabular}{lrrrrrrr}
\toprule
& \multicolumn{7}{c}{Dose scale $\alpha$} \\
\cmidrule(lr){2-8}
Simulator ($\tau$) & 0 & 0.25 & 0.5 & 1 & 1.5 & 2 & 4 \\
\midrule
World model ($\tau{=}4$) & \emph{0.893} & 0.312 & 0.310 & 0.310 & 0.311 &
0.311 & 0.316 \\
Pooled-hazard GBM ($\tau{=}4$) & \emph{0.632} & 0.315 & 0.314 & 0.313 &
0.318 & 0.325 & 0.364 \\
World model ($\tau{=}8$) & \emph{0.708} & 0.267 & 0.265 & 0.265 & 0.266 &
0.267 & 0.270 \\
Pooled-hazard GBM ($\tau{=}8$) & \emph{0.504} & 0.273 & 0.272 & 0.271 &
0.275 & 0.279 & 0.307 \\
\bottomrule
\end{tabular}
\end{table}

Task (T3) is the capability that neither per-horizon classifiers nor
outcome-only hazard models have: from a cutoff $\tau$, replace the future
exposures with a stated scenario $\ba'$, re-roll the model, and read off
the change in the predicted conversion trajectory. We ran overall dose
scaling $\ba' = \alpha\,\ba$ with $\alpha \in \{0, 0.25, 0.5, 1, 1.5, 2,
4\}$, per-channel and per-targeting-lever shutoffs, and a placebo control
(scaling a negligible exposure bucket by $4\times$), at $\tau \in \{4,
8\}$ on the dx outcome. As a reference simulator we also perturbed the
pooled-hazard GBM's future exposure features. Table~\ref{tab:exp3} shows
the dose-response; the reading comes in three parts, and the honest part
is the most interesting one.

\paragraph{Within the observed support, the simulation is sane but small.}
For $\alpha \in [0.25, 2]$, holding the weekly activity pattern fixed and
scaling the exposure magnitudes, the world model's dose-response is
monotone and saturating, moving by about $+0.6$ percentage points for a
$4\times$ dose increase (0.310 to 0.316 at $\tau = 4$). The placebo
scenario moves the forecast by less than $10^{-4}$, and every single-lever
shutoff moves it by at most 0.003. So the simulator passes its negative
controls and finds little marginal effect of exposure \emph{intensity} ---
a plausible answer on targeting-driven data, where whom the campaign
reaches plausibly matters more than how hard it re-reaches them.

\paragraph{Off the support, the simulation exposes the data, not the
model.} The $\alpha = 0$ scenario --- switch all future exposure off ---
should, on a causal reading, produce the \emph{lowest} conversion. It
produces the highest by far: 0.89 at $\tau = 4$ against 0.31 at $\alpha =
1$. The mechanism is selection through censoring: in the observed data a
patient's exposure stops once they convert, so ``no future exposure'' is,
to the model, strong evidence of imminent conversion. The pooled-hazard
GBM shows the same inversion (0.63), so this is a property of
observational exposure data under outcome-dependent censoring, not a
defect of one architecture. We report this number prominently on purpose.
It is a concrete, quantified demonstration of the warning in
Section~\ref{sec:problem}: an exposure-conditioned simulator answers
``what do patients who look like this do?'', and off the data's support
that question silently diverges from ``what would happen if we did
this?''.

\paragraph{What survives.} The capability is real --- one model produces
per-patient, action-conditioned trajectories under any stated plan, which
is the input a media planner actually wants --- but on this data its
outputs are decision-support signals under stated assumptions, not effect
estimates. Turning them into effects requires design: holdouts,
randomization, or explicit deconfounding \citep{robins2000,kunzel2019},
plus support checks of the kind that flagged $\alpha = 0$ and $\alpha = 4$
here. A cleaner protocol variant (holding the activity flag fixed at
$\alpha = 0$, restricting reports to the observed dose support) is noted
in Appendix~\ref{app:exp3}.

\section{What this means in practice}
\label{sec:practice}

The three findings compress into three pieces of advice for teams that
measure campaigns in flight.

\textbf{1. Fix the formulation first.} Most of the gap between common
practice and the world model is closed by the survival-rollout structure
alone, which any pooled-hazard model can wear, including the GBM a team
already has. If a measurement stack trains one classifier per
cutoff-horizon cell, the cheapest upgrade is not a deep model; it is a
pooled hazard and a product formula.

\textbf{2. Buy the learned state when the regime calls for it.} On sparse
histories and a common outcome, a well-calibrated GBM hazard is nearly as
good as the world model at the aggregate level; the world model's constant
$+0.02$ AUROC is worth it only if patient-level ranking feeds decisions.
The regimes that justify the sequence model are rare outcomes (here,
$5$--$41\times$ lower volume error on rx) and patients with real exposure
dynamics ($2$--$10\times$ on the active subgroup) --- and these are exactly
the regimes a one-page Fisher calculation identifies before any training
run.

\textbf{3. Simulate for planning, not for effect estimation.} The
transition model turns the forecaster into a simulator, and the simulator
is useful --- it answers ``what does the model expect under this plan?''
coherently, per patient, for any plan. But on targeting-driven data its
extreme scenarios measure selection, not response, and the $\alpha = 0$
inversion in Table~\ref{tab:exp3} is what that failure looks like at full
size. Scenario outputs should ship with support flags and negative
controls, and effect claims should wait for design.

\section{Limitations}
\label{sec:limitations}

\textbf{Observational exposure.} Delivery is targeted, not randomized, so
confounding between exposure intensity and the latent propensity to
convert is expected, and Section~\ref{ssec:exp3} shows it is not
hypothetical. All forecasts are exposure-conditioned; no causal claims are
made. \textbf{Enriched cohort.} The 33.6\% training prevalence is a design
choice, corrected at evaluation with inverse-sampling weights; the
IPW-corrected metrics are the ones that carry over to the real population.
\textbf{Sequence sparsity.} With a median of three active weeks per
patient, the full-cohort dx results likely understate what the model would
do on denser campaigns; the dynamics-rich subgroup is our best in-data
proxy for that setting, and it is one fifth of the cohort.
\textbf{Transition supervision.} Its measured value for \emph{passive}
forecasting is confined to the rare-outcome regime (rx volume); on dx it
is neutral. Its unconditional value is that it enables (T3) at all.
\textbf{Tail cutoffs.} At $\tau = 39$ the risk sets have few future
converters (631 on dx, 76 on rx) and all volume errors there are noisy;
we present them and do not interpret their ordering. \textbf{Single
campaign.} All results come from one campaign, one therapeutic area, one
country. External validity is untested. \textbf{Known-exposure rollout.}
The T2 evaluation feeds the recorded future exposures to every model,
isolating response dynamics from media-plan forecasting; an operational
forecast would add a stated future plan, whose uncertainty is out of scope
here.

\section{Conclusion}
\label{sec:concl}

This paper set out to answer a question benchmarks alone do not: when a
patient world model is applied to in-flight campaign measurement, which
ingredient earns its keep? The formulation --- a discrete-time survival
hazard rolled out from a latent state --- turned out to be the workhorse:
it is what replaces hundreds-of-percent volume errors with single digits,
and it costs nothing beyond a change of target. The learned recurrent
state earns its keep in the regimes a short Fisher-information argument
predicts: rare outcomes and dynamics-rich patients, where it cuts volume
error by up to $40\times$ over a strong coherent baseline. The transition
model earns its keep twice: once as dense supervision exactly where
outcome labels run out, and once as the machinery of scenario simulation
--- whose sharpest output here was an honest one, a quantified
demonstration that off-support counterfactuals on targeted exposure data
measure selection rather than response. We believe this anatomy ---
structure first, learned state where theory says it pays, simulation with
guardrails --- is the right way to bring world models into observational
health-outcomes measurement, and the recipe applies wherever longitudinal
exposures meet sparse terminal outcomes: adherence programs, vaccination
campaigns, and public-health communication among them.

\paragraph{Reproducibility and data availability.} The underlying data
are protected health information and cannot be shared. All reported
numbers are aggregate metrics computed inside a certified analytics
environment. Cohort construction rules, feature definitions, and
hyperparameters are given in
Appendices~\ref{app:cohort}--\ref{app:exp3}, at a level of detail
sufficient to rebuild the pipeline on comparable data.

\bibliographystyle{plainnat}
\bibliography{refs}

\appendix

\section{Cohort construction}
\label{app:cohort}

The modeling universe contains 10.88M patients with campaign eligibility.
The stratified case-control cohort keeps: all rx converters (5{,}225), all
on-market comparator patients (4{,}399), a deterministic-hash subsample of
dx converters (44{,}917), and a deterministic-hash subsample of on-market
non-converting negatives with at least eight observed weeks (95{,}061).
The total is 147{,}173 patients. Deterministic hashing (no random seed)
makes the cohort exactly reproducible from the universe. Each patient
carries $w_i = 1/(\text{stratum sampling fraction})$, equal to 1 for the
kept-all strata. Evaluation-time inverse-probability weighting with $w_i$
restores natural prevalence \citep{horvitz1952}.

Calendar weeks are indexed as $\mathrm{wk} =
\lfloor(\text{date} - \text{2024-01-01})/7\rfloor$; the relative week is
$r = \mathrm{wk} - \mathrm{wk}_{\text{index}}$. The observation horizon is
$r \in [0, 52]$ with a fixed absolute window end, so each patient's
observed relative window is $\min(52,\; 53 - \mathrm{wk}_{\text{index}})$.
Late enrollers have shorter windows, and this is handled as
right-censoring in the survival likelihood. After a conversion event the
patient exits the risk set. Splits are 70/15/15 by patient hash; no
patient appears in more than one split. The dynamics-rich subgroup used in
Section~\ref{ssec:exp2q2} is defined as patients with at least five total
active exposure weeks over the window (29{,}859 patients, 20.3\%); the
originally intended ``$\ge 8$ active weeks'' definition is nearly empty
under this cohort's sparsity and was widened before any model comparison
was made on the subgroup.

\section{Feature definitions}
\label{app:features}

\paragraph{Per-week action vector ($d_a = 17$).} \texttt{imp\_log}
($\log(1+x)$ of the p99-winsorized total weekly impressions);
$\log(1+\cdot)$ of the weekly event count; $\log(1+\cdot)$ impression
volumes in three channel buckets (digital, programmatic, display); three
ad-type buckets (display, video, audio); seven targeting buckets
(condition, lookalike, behavioral-contextual, conquesting, retargeting,
geo-demographic, none/other); a week-active flag; and the normalized
relative week $r/52$.

\paragraph{Static vector ($d_s = 7$).} Source-of-business one-hot (three
levels: market-naive, switched from another product, continuing on brand),
rx-eligibility flag, dx-eligibility flag, $\log(1+\cdot)$ prior
office-visit count, and normalized enrollment week.

\paragraph{Survival convention.} The hazard emitted from state $\bz_{i,r}$
predicts an event in week $r{+}1$. At-risk person-weeks are pooled for
training and evaluation. Patients are censored at their observation end.

\section{Training details}
\label{app:training}

The proposed model is implemented in PyTorch and trained on CPU. The tuned
configuration (selected on validation hazard likelihood) uses two GRU
layers, hidden size 128, dropout 0.2; the base configuration is one layer,
hidden size 64. Task (T1) results (Table~\ref{tab:exp1}) are from the base
configuration; the rollout and simulation experiments use the tuned
configuration. The static projection $W_0$ maps the static vector to the
initial hidden state of every layer. The hazard head is $\mathrm{hidden}
\to \mathrm{hidden} \to 1$ with ReLU and dropout; the transition head maps
$(\bz_{i,r}, \ba_{i,r})$ through one hidden layer to the 17-dimensional
next-week action summary. The loss weight is $\lambda = 0.3$.
Optimization: Adam, learning rate $10^{-3}$, \texttt{ReduceLROnPlateau}
(factor 0.5, patience 2) on validation hazard negative log-likelihood,
early stopping (patience 10), at most 50 epochs, batch size 512. A control
run at batch size 1024 produced materially identical results, so batch
size is not a sensitive choice here. The GRU forecaster ablation sets
$\lambda = 0$ and removes the transition head; nothing else changes. On
the rollout task the transition head reaches $+11.5\%$ held-out skill over
the training-mean predictor (on both outcomes). Baselines use standard
library defaults (scikit-learn for logistic regression and MLP; LightGBM
\citep{ke2017} for all GBM variants) and are reported as-run.

\section{Scenario-simulation details}
\label{app:exp3}

The simulator is the tuned world model (45 epochs, otherwise as in
Appendix~\ref{app:training}), applied to the full test risk sets at $\tau
\in \{4, 8\}$ on the dx outcome. Dose scaling multiplies all future
exposure magnitudes by $\alpha$; at $\alpha = 0$ this also zeroes the
week-active flag, which is what triggers the selection artifact discussed
in Section~\ref{ssec:exp3}. Per-lever shutoffs zero one action dimension's
future values (13 levers: channel, ad-type, and targeting buckets); the
largest observed shift was $+0.0026$ (total digital volume off), and the
placebo lever moved the forecast by less than $10^{-4}$. Per-patient
dose-response monotonicity (over all $\alpha$, including 0) holds for
20--29\% of patients, dragged down by the $\alpha = 0$ artifact. Two
protocol refinements are noted for future runs: hold the week-active
pattern fixed at $\alpha = 0$ so that only magnitude varies, and restrict
reported curves to the observed dose support (approximately $\alpha \in
[0.25, 2]$).

